Decade-long Utilization Patterns of ICSE Technical Papers and Associated Artifacts

Context: Annually, ICSE acknowledges a range of papers, a subset of which are paired with research artifacts such as source code, datasets, and supplementary materials, adhering to the Open Science Policy. However, no prior systematic inquiry dives into gauging the influence of ICSE papers using artifact attributes. Objective: We explore the mutual impact between artifacts and their associated papers presented at ICSE over ten years. Method: We collect data on usage attributes from papers and their artifacts, conduct a statistical assessment to identify differences, and analyze the top five papers in each attribute category. Results: There is a significant difference between paper citations and the usage of associated artifacts. While statistical analyses show no notable difference between paper citations and GitHub stars, variations exist in views and/or downloads of papers and artifacts. Conclusion: We provide a thorough overview of ICSE's accepted papers from the last decade, emphasizing the intricate relationship between research papers and their artifacts. To enhance the assessment of artifact influence in software research, we recommend considering key attributes that may be present in one platform but not in another.

==> res/tbl/tbl_metric_pvalue.tex <==


\begin{table}[htbp]
\caption{Paired T-Test on Paper and Artifact Attributes}
\footnotesize{
Here, $\ast$: p-value < 0.05 ,$\ast$$\ast$: p-value < 0.01
,  $\ast$$\ast$$\ast$: p-value < 0.001 
}
\label{tbl_metrics_p}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{0.3\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}|}
\hline
Attributes &   Normalized paper citations& Normalized overall artifact usage \\ \hline
has-discussion       & $\ast$$\ast$$\ast$      & $\ast$$\ast$$\ast$        \\ \hline

\#issues-open        & ---            & $\ast$$\ast$$\ast$        \\ \hline

\#issues-closed      & ---           & $\ast$$\ast$$\ast$        \\ \hline

longest-issue        & $\ast$        & $\ast$$\ast$$\ast$        \\ \hline

number-of-commits   & $\ast$         & $\ast$               \\ \hline

last-commit-date    & $\ast$$\ast$$\ast$      & $\ast$$\ast$$\ast$        \\ \hline

stars                 & $\ast$$\ast$$\ast$      & $\ast$$\ast$$\ast$     \\ \hline

watching              & ---            & $\ast$$\ast$$\ast$        \\ \hline

forks                 & ---            & $\ast$$\ast$$\ast$        \\ \hline

artifact-downloads    & $\ast$         & ---              \\ \hline

artifact-views        & $\ast$$\ast$$\ast$  & $\ast$$\ast$$\ast$     \\ \hline

paper-views/downloads & $\ast$$\ast$$\ast$     & $\ast$$\ast$$\ast$     \\ \hline

paper-citation counts       & $\ast$$\ast$$\ast$      & $\ast$$\ast$$\ast$     \\ \hline
\end{tabular}%
}
% \caption*{ 
% p-value < 0.05 == $\ast$

% p-value < 0.01 == $\ast$$\ast$

% p-value < 0.001 == $\ast$$\ast$$\ast$
% }
\end{table}



% \begin{table}[]
% \caption{}
% \label{tab:my-table}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{Metric} & Paired t-test normalize paper citation & \multicolumn{1}{l|}{Paired t-test normalize usage count} \\ \hline
% has\_discussion       & 5.46E-13      & 8.88E-09        \\ \hline
% \#issues\_open        & 0.133730847   & 6.76E-07        \\ \hline
% \#issues\_closed      & 0.1926818924  & 2.18E-06        \\ \hline
% longest\_issue        & 0.03321542125 & 6.16E-07        \\ \hline
% number\_of\_commits   & 0.02542780302 & 0.04268689677   \\ \hline
% last\_commit\_date    & 5.80E-14      & 3.56E-10        \\ \hline
% stars                 & 3.02E-08      & 0.0005056592969 \\ \hline
% watching              & 0.4863523719  & 1.04E-06        \\ \hline
% forks                 & 0.0686128277  & 2.13E-15        \\ \hline
% artifact-downloads    & 0.01664333423 & 0.101427439     \\ \hline
% artifact-views        & 8.12E-05      & 0.0003502252613 \\ \hline
% paper-views/downloads & 3.30E-30      & 1.04E-23        \\ \hline
% paper-citations       & 1.04E-12      & 8.74E-06        \\ \hline
% \end{tabular}%
% }
% \end{table

==> res/tbl/tbl_metrics.tex <==
\begin{table*}[hbtp]
\caption{Top Five Papers for Usage Attributes}
\label{tbl_top5_papers}
% \renewcommand{\arraystretch}{.85}

\resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|l|c|c|}
\begin{tabular}{|p{0.17\linewidth}|p{0.04\linewidth}|p{0.80\linewidth}|p{0.04\linewidth}|}
\hline
\textbf{Attribute} & \textbf{ID} & \textbf{Paper Title} & \textbf{Value} \\ \hline
\multirow{5}{*}{\#issues-open} & 58 & Feedback-Based Debugging & 54 \\ \cline{2-4} 
 & 145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams & 48 \\ \cline{2-4} 
 & 68 & Automated Refactoring of Legacy Java Software to Default Methods & 47 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 34 \\ \cline{2-4} 
 & 2 & Building and Using Pluggable Type-Checkers & 33 \\ \hline
\multirow{5}{*}{stars} & 135 & Guiding Deep Learning System Testing using Surprise Adequacy & 365 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 289 \\ \cline{2-4} 
 & 83 & Deep Code Search & 266 \\ \cline{2-4} 
 & 218 & Interface Compliance of Inline Assembly: Automatically Check, Patch and Refine & 244 \\ \cline{2-4} 
 & 46 & Termination-Checking for LLVM Peephole Optimizations & 210 \\ \hline
\multirow{5}{*}{watching} & 135 & Guiding Deep Learning System Testing using Surprise Adequacy & 35 \\ \cline{2-4} 
 & 35 & On Architectural Diversity of Dynamic Adaptive Systems & 20 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 19 \\ \cline{2-4} 
 & 38 & DoubleTake: Fast and Precise Error Detection via Evidence-Based Dynamic Analysis & 18 \\ \cline{2-4} 
 & 46 & Termination-Checking for LLVM Peephole Optimizations & 16 \\ \hline
\multirow{5}{*}{forks} & 10 & Understanding Integer Overflow in C/C++ & 1700 \\ \cline{2-4} 
 & 35 & On Architectural Diversity of Dynamic Adaptive Systems & 1400 \\ \cline{2-4} 
 & 59 & How Do Developers Fix Cross-Project Correlated Bugs? A Case Study on the GitHub Scientific Python Ecosystem & 214 \\ \cline{2-4} 
 & 135 & Guiding Deep Learning System Testing using Surprise Adequacy & 140 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 121 \\ \hline
\multirow{5}{*}{\#issues-closed} & 99 & Accurate and Efficient Refactoring Detection in Commit History & 355 \\ \cline{2-4} 
 & 58 & Feedback-Based Debugging & 180 \\ \cline{2-4} 
 & 68 & Automated Refactoring of Legacy Java Software to Default Methods & 113 \\ \cline{2-4} 
 & 2 & Building and Using Pluggable Type-Checkers & 108 \\ \cline{2-4} 
 & 145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams & 78 \\ \hline
\multirow{5}{*}{longest-issue} & 145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams & 73 \\ \cline{2-4} 
 & 68 & Automated Refactoring of Legacy Java Software to Default Methods & 42 \\ \cline{2-4} 
 & 83 & Deep Code Search & 21 \\ \cline{2-4} 
 & 148 & The List is the Process: Reliable Pre-Integration Tracking of Commits on Mailing Lists & 20 \\ \cline{2-4} 
 & 132 & Gigahorse: Thorough, Declarative Decompilation of Smart Contracts & 15 \\ \hline
\multirow{5}{*}{\#pull-requests-open} & 143 & Reasonably-Most-General Clients for JavaScript Library Analysis & 20 \\ \cline{2-4} 
 & 50 & Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game & 10 \\ \cline{2-4} 
 & 58 & Feedback-Based Debugging & 9 \\ \cline{2-4} 
 & 181 & Near-Duplicate Detection in Web App Model Inference & 7 \\ \cline{2-4} 
 & 52 & PEoPL: Projectional Editing of Product Lines & 6 \\ \hline
\multirow{5}{*}{\#pull-requests-closed} & 2 & Building and Using Pluggable Type-Checkers & 472 \\ \cline{2-4} 
 & 202 & Verifying Object Construction & 455 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 87 \\ \cline{2-4} 
 & 33 & MU-MMINT: An IDE for Model Uncertainty & 85 \\ \cline{2-4} 
 & 132 & Gigahorse: Thorough, Declarative Decompilation of Smart Contracts & 83 \\ \hline
\multirow{5}{*}{longest-pull-request} & 148 & The List is the Process: Reliable Pre-Integration Tracking of Commits on Mailing Lists & 125 \\ \cline{2-4} 
 & 202 & Verifying Object Construction & 99 \\ \cline{2-4} 
 & 145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams & 63 \\ \cline{2-4} 
 & 209 & Data-Oriented Differential Testing of Object-Relational Mapping Systems & 35 \\ \cline{2-4} 
 & 73 & Search-Based Test Data Generation for SQL Queries & 21 \\ \hline
\multirow{5}{*}{number-of-contributors} & 2 & Building and Using Pluggable Type-Checkers & 27 \\ \cline{2-4} 
 & 10 & Understanding Integer Overflow in C/C++ & 27 \\ \cline{2-4} 
 & 132 & Gigahorse: Thorough, Declarative Decompilation of Smart Contracts & 18 \\ \cline{2-4} 
 & 35 & On Architectural Diversity of Dynamic Adaptive Systems & 16 \\ \cline{2-4} 
 & 50 & Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game & 16 \\ \hline
\multirow{5}{*}{number-of-commits} & 10 & Understanding Integer Overflow in C/C++ & 40162 \\ \cline{2-4} 
 & 50 & Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game & 4464 \\ \cline{2-4} 
 & 33 & MU-MMINT: An IDE for Model Uncertainty & 3295 \\ \cline{2-4} 
 & 2 & Building and Using Pluggable Type-Checkers & 2290 \\ \cline{2-4} 
 & 99 & Accurate and Efficient Refactoring Detection in Commit History & 2054 \\ \hline
\multirow{5}{*}{artifact-downloads} & 170 & Heaps'n Leaks: How Heap Snapshots Improve Android Taint Analysis & 8388 \\ \cline{2-4} 
 & 233 & SOAR: A Synthesis Approach for Data Science API Refactoring & 3343 \\ \cline{2-4} 
 & 228 & Representation of Developer Expertise in Open Source Software & 2553 \\ \cline{2-4} 
 & 212 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests & 1410 \\ \cline{2-4} 
 & 18 & Data clone detection and visualization in spreadsheets & 849 \\ \hline
\multirow{5}{*}{artifact-views} & 122 & Automated Reporting of Anti-Patterns and Decay in Continuous Integration & 5463 \\ \cline{2-4} 
 & 18 & Data clone detection and visualization in spreadsheets & 1998 \\ \cline{2-4} 
 & 103 & A Large-Scale Empirical Study on the Effects of Code Obfuscations on Android Apps and Anti-Malware Products & 1417 \\ \cline{2-4} 
 & 150 & The Seven Sins: Security Smells in Infrastructure as Code Scripts & 995 \\ \cline{2-4} 
 & 212 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests & 846 \\ \hline
\multirow{5}{*}{paper-views/downloads} & 121 & A Novel Neural Source Code Representation based on Abstract Syntax Tree & 5704 \\ \cline{2-4} 
 & 12 & Where should the bugs be fixed? More accurate information retrieval-based bug localization based on bug reports & 3513 \\ \cline{2-4} 
 & 71 & Semantically Enhanced Software Traceability Using Deep Learning Techniques & 3067 \\ \cline{2-4} 
 & 230 & Semi-supervised Log-based Anomaly Detection via Probabilistic Label Estimation & 2343 \\ \cline{2-4} 
 & 106 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars & 2218 \\ \hline
\multirow{5}{*}{paper-citations} & 106 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars & 321 \\ \cline{2-4} 
 & 12 & Where should the bugs be fixed? More accurate information retrieval-based bug localization based on bug reports & 317 \\ \cline{2-4} 
 & 135 & Guiding Deep Learning System Testing using Surprise Adequacy & 166 \\ \cline{2-4} 
 & 121 & A Novel Neural Source Code Representation based on Abstract Syntax Tree & 153 \\ \cline{2-4} 
 & 83 & Deep Code Search & 134 \\ \hline
\end{tabular}%
}
\end{table*}

==> res/tbl/tbl_metrics_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%\begin{table*}[]
%\caption{}
%\label{tab:my-table}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|l|c|c|}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[hbtp]
\caption{Top Five Papers for Usage Attributes}
\label{tbl_top5_papers}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|l|c|c|}
\begin{tabular}{|p{0.04\linewidth}|p{0.80\linewidth}|p{0.175\linewidth}|p{0.04\linewidth}|}
\hline
% \multicolumn{1}{|l|}{Paper ID} &
%   \multicolumn{1}{c|}{\textbf{Paper Title}} &
%   \textbf{Metric} &
%   \multicolumn{1}{l|}{\textbf{Metric Value}} \\ \hline
\textbf{ID} &
\textbf{Paper Title }&
\textbf{Attribute} &
\textbf{Value} \\ \hline
% 1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Longest Issue                          & 73    \\ \hline
% 1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Issues Open                            & 48    \\ \hline
% 1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Issues Closed                          & 78    \\ \hline
% 2  & Automated Refactoring of Legacy Java Software to Default Methods                    & Longest Issue                          & 42    \\ \hline
% 2  & Automated Refactoring of Legacy Java Software to Default Method                     & Issues Open                            & 47    \\ \hline
% 2  & Automated Refactoring of Legacy Java Software to Default Methods                    & Issues Closed                          & 112   \\ \hline
% 3  & Learning Syntactic Program Transformations from Examples                            & Longest Issue                          & 24    \\ \hline
% 4  & Deep Code Search                                                                    & Stars                                  & 266   \\ \hline
% 4  & Deep Code Search                                                                    & Paper Citations                        & 134   \\ \hline
% 4  & Deep Code Search                                                                    & Longest Issue                          & 21    \\ \hline
% 5 &
%   The List is the Process: Reliable Pre-Integration Tracking of Commits on Mailing Lists &
%   Longest Issue &
%   20 \\ \hline
% 6  & Feedback-Based Debugging                                                            & Issues Open                            & 54    \\ \hline
% 6  & Feedback-Based Debugging                                                            & Issues Closed                          & 180   \\ \hline
% 7  & Accurate and Efficient Refactoring Detection in Commit History                      & Issues Open                            & 34    \\ \hline
% 7  & Accurate and Efficient Refactoring Detection in Commit History                      & Forks                                  & 121   \\ \hline
% 7  & Accurate and Efficient Refactoring Detection in Commit History                      & Issues Closed                          & 355   \\ \hline
% 7  & Accurate and Efficient Refactoring Detection in Commit History                      & Watching                               & 19    \\ \hline
% 7  & Accurate and Efficient Refactoring Detection in Commit History                      & Stars                                  & 289   \\ \hline
% 8  & Building and Using Pluggable Type-Checkers                                          & Issues Open                            & 33    \\ \hline
% 8  & Building and Using Pluggable Type-Checkers                                          & \\#Commits & 2290  \\ \hline
% 8  & Building and Using Pluggable Type-Checkers                                          & Issues Closed                          & 108   \\ \hline
% 9  & Understanding Integer Overflow in C/C++                                             & Forks                                  & 1700  \\ \hline
% 9  & Understanding Integer Overflow in C/C++                                             & \\#Commits & 40162 \\ \hline
% 10 & Reducer-Based Construction of Conditional Verifiers                                 & \\#Commits & 32527 \\ \hline
% 10 & Reducer-Based Construction of Conditional Verifiers                                 & Watching                               & 21    \\ \hline
% 11 &
%   Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game &
%   \\#Commits &
%   4464 \\ \hline
% 12 & MU-MMINT: An IDE for Model Uncertainty                                              & \\#Commits & 3295  \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Forks                                  & 140   \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Watching                               & 35    \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Stars                                  & 365   \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Paper Citations                        & 166   \\ \hline
% 14 & On Architectural Diversity of Dynamic Adaptive Systems                              & Watching                               & 20    \\ \hline
% 14 & On Architectural Diversity of Dynamic Adaptive Systems                              & Forks                                  & 1400  \\ \hline
% 15 & DoubleTake: Fast and Precise Error Detection via Evidence-Based Dynamic Analysis    & Watching                               & 18    \\ \hline
% 16 & How Do Developers Fix Cross-Project Correlated Bugs? A Case Study on the GitHub ... & Forks                                  & 214   \\ \hline
% 17 & Interface Compliance of Inline Assembly: Automatically Check, Patch and Refine      & Stars                                  & 244   \\ \hline
% 18 & Termination-Checking for LLVM Peephole Optimizations                                & Stars                                  & 210   \\ \hline
% 19 & Heaps'n Leaks: How Heap Snapshots Improve Android Taint Analysis                    & Artifact Downloads                     & 8388  \\ \hline
% 20 & SOAR: A Synthesis Approach for Data Science API Refactoring                         & Artifact Downloads                     & 3343  \\ \hline
% 21 & Representation of Developer Expertise in Open Source Software                       & Artifact Downloads                     & 2553  \\ \hline
% 22 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                          & Artifact Downloads                     & 1410  \\ \hline
% 22 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                          & Artifact Views                         & 846   \\ \hline
% 23 & Data clone detection and visualization in spreadsheets                              & Artifact Downloads                     & 849   \\ \hline
% 24 & Automated Reporting of Anti-Patterns and Decay in Continuous Integration            & Artifact Views                         & 5463  \\ \hline
% 25 & Data clone detection and visualization in spreadsheets                              & Artifact Views                         & 1998  \\ \hline
% 26 & Learning from, Understanding, and Supporting DevOps Artifacts for Docker            & Artifact Views                         & 712   \\ \hline
% 27 & Recognizing Developers' Emotions while Programming                                  & Artifact Views                         & 667   \\ \hline
% 28 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars           & Paper Citations                        & 321   \\ \hline
% 28 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars           & Paper Views                            & 2218  \\ \hline
% 29 & A Novel Neural Source Code Representation based on Abstract Syntax Tree             & Paper Citations                        & 153   \\ \hline
% 29 & A Novel Neural Source Code Representation based on Abstract Syntax Tree             & Paper Views                            & 5704  \\ \hline
% 30 & Semantically Enhanced Software Traceability Using Deep Learning Techniques          & Paper Citations                        & 132   \\ \hline
% 30 & Semantically Enhanced Software Traceability Using Deep Learning Techniques          & Paper Views                            & 3067  \\ \hline
% 31 & Semi-supervised Log-based Anomaly Detection via Probabilistic Label Estimation      & Paper Views                            & 2343  \\ \hline
% 32 & Measuring Program Comprehension: A Large-Scale Field Study with Professionals       & Paper Views                            & 2086  \\ \hline

145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams                                & Issues Closed      & 78    \\  \hline
145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams                                & Issues Open        & 48    \\  \hline
145 & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams                                & \textbf{Longest Issue }     & \textbf{73}    \\  \hline
67  & Automated Refactoring of Legacy Java Software to Default Methods                                            & Issues Closed      & 113   \\  \hline
67  & Automated Refactoring of Legacy Java Software to Default Methods                                             & Issues Open        & 47    \\  \hline
67  & Automated Refactoring of Legacy Java Software to Default Methods                                            & Longest Issue      & 42    \\  \hline
%56  & Learning Syntactic Program Transformations from Examples                                                    & Longest Issue      & 24    \\  \hline
131  & Gigahorse: Thorough, Declarative Decompilation of Smart Contracts	                                                    & Longest Issue      & 15    \\  \hline
82  & Deep Code Search                                                                                            & Longest Issue      & 21    \\  \hline
82  & Deep Code Search                                                                                            & Paper Citations    & 134   \\  \hline
82  & Deep Code Search                                                                                            & Stars              & 266   \\  \hline
148 & The List is the Process: Reliable Pre-Integration Tracking of Commits on Mailing Lists                      & Longest Issue      &   20    \\  \hline
57  & Feedback-Based Debugging                                                                                    & Issues Closed      & 180   \\  \hline
57  & Feedback-Based Debugging                                                                                    & \textbf{Issues Open}        & \textbf{54}    \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & Forks              & 121   \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & \textbf{Issues Closed }     & \textbf{355}   \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & Issues Open        & 34    \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & Stars              & 289   \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & Watching           & 19    \\  \hline
99  & Accurate and Efficient Refactoring Detection in Commit History                                              & \#Commits           & 2054    \\  \hline
1   & Building and Using Pluggable Type-Checkers                                                                  & \#Commits           & 2290  \\  \hline
1   & Building and Using Pluggable Type-Checkers                                                                  & Issues Closed      & 108   \\  \hline
1   & Building and Using Pluggable Type-Checkers                                                                  & Issues Open        & 33    \\  \hline
9   & Understanding Integer Overflow in C/C++                                                                     & \textbf{\#Commits}           & \textbf{40162} \\
\hline
9   & Understanding Integer Overflow in C/C++                                                                     & \textbf{Forks}              & \textbf{1700}  \\  \hline
%73  & Reducer-Based Construction of Conditional Verifiers                                                         & \#Commits           & 32527 \\
%73  & Reducer-Based Construction of Conditional Verifiers                                                         & Watching           & 21    \\  \hline
49  & Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game               & \#Commits           &   4464    \\  \hline
32  & MU-MMINT: An IDE for Model Uncertainty                                                                      & \#Commits           & 3295  \\  \hline
135 & Guiding Deep Learning System Testing using Surprise Adequacy                                                & Forks              & 140   \\  \hline
135 & Guiding Deep Learning System Testing using Surprise Adequacy                                                & Paper Citations    & 166   \\  \hline
135 & Guiding Deep Learning System Testing using Surprise Adequacy                                                & \textbf{Stars}              & \textbf{365}   \\  \hline
135 & Guiding Deep Learning System Testing using Surprise Adequacy                                                & \textbf{Watching}           & \textbf{35}    \\  \hline
34  & On Architectural Diversity of Dynamic Adaptive Systems                                                      & Forks              & 1400  \\  \hline
34  & On Architectural Diversity of Dynamic Adaptive Systems                                                      & Watching           & 20    \\  \hline
37  & DoubleTake: Fast and Precise Error Detection via Evidence-Based Dynamic Analysis                            & Watching           & 18    \\  \hline
58  & How Do Developers Fix Cross-Project Correlated Bugs? A Case Study on the GitHub Scientific Python Ecosystem & Forks              & 214   \\  \hline
218 & Interface Compliance of Inline Assembly: Automatically Check, Patch and Refine                              & Stars              & 244   \\  \hline
45  & Termination-Checking for LLVM Peephole Optimizations                                                        & Stars              & 210   \\  \hline
45  & Termination-Checking for LLVM Peephole Optimizations                                                        & Watching              & 16   \\  \hline
170 & Heaps'n Leaks: How Heap Snapshots Improve Android Taint Analysis                                            & \textbf{Artifact Downloads} & \textbf{8388}  \\  \hline
233 & SOAR: A Synthesis Approach for Data Science API Refactoring                                                 & Artifact Downloads & 3343  \\  \hline
228 & Representation of Developer Expertise in Open Source Software                                               & Artifact Downloads & 2553  \\  \hline
212 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                                                  & Artifact Downloads & 1410  \\  \hline
212 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                                                  & Artifact Views     & 846   \\  \hline
17  & Data clone detection and visualization in spreadsheets                                                      & Artifact Downloads & 849   \\  \hline
17  & Data clone detection and visualization in spreadsheets                                                      & Artifact Views     & 1998  \\  \hline
122 & Automated Reporting of Anti-Patterns and Decay in Continuous Integration                                    & \textbf{Artifact Views }    & \textbf{5463}  \\  \hline
%176 & Learning from, Understanding, and Supporting DevOps Artifacts for Docker                                    & Artifact Views     & 712   \\  \hline
%189 & Recognizing Developers' Emotions while Programming                                                          & Artifact Views     & 667   \\  \hline
106 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars                                   & \textbf{Paper Citations }   & \textbf{321}   \\  \hline
106 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars                                   & Paper Views        & 2218  \\  \hline
121 & A Novel Neural Source Code Representation based on Abstract Syntax Tree                                     & Paper Citations    & 153   \\  \hline
121 & A Novel Neural Source Code Representation based on Abstract Syntax Tree                                     & \textbf{Paper Views }       & \textbf{5704}  \\  \hline
70  & Semantically Enhanced Software Traceability Using Deep Learning Techniques                                  & Paper Citations    & 132   \\  \hline
70  & Semantically Enhanced Software Traceability Using Deep Learning Techniques                                  & Paper Views        & 3067  \\  \hline
230 & Semi-supervised Log-based Anomaly Detection via Probabilistic Label Estimation                              & Paper Views        & 2343  \\  \hline
93  & Measuring Program Comprehension: A Large-Scale Field Study with Professionals                               & Paper Views        & 2086 \\ \hline
102  & A Large-Scale Empirical Study on the Effects of Code Obfuscations on Android Apps and Anti-Malware Products  & Artifact Views        & 1417 \\ \hline
149  & The Seven Sins: Security Smells in Infrastructure as Code Scripts      & 
Artifact Views        & 995 \\ \hline

\end{tabular}%
} 
\footnotesize{ Here, attribute and values are in bold denote the highest number for each attribute.}
\end{table*}

==> res/tbl/tbl_pl_pvalue.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htbp]
\caption{Paired t-test  (Normalized)}
\footnotesize{
Here, $\ast$: p-value < 0.05 ,$\ast$$\ast$: p-value < 0.01
,  $\ast$$\ast$$\ast$: p-value < 0.001 
}
\label{tbl_pl_pvalue}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Programming Language}} & \textbf{paper citation} & \multicolumn{1}{l|}{\textbf{usage count}} \\ \hline
Scala      & $\ast$$\ast$            & ---  \\ \hline
C++        & $\ast$$\ast$$\ast$      & --- \\ \hline
JavaScript & $\ast$$\ast$$\ast$      & --- \\ \hline
HTML       & $\ast$$\ast$            & --- \\ \hline
OCamel     & $\ast$$\ast$$\ast$      & $\ast$ \\ \hline
Shell      & ---                     & $\ast$ \\ \hline
MATLAB     & ---                     & $\ast$ \\ \hline
Other      & $\ast$$\ast$            & $\ast$$\ast$$\ast$            \\ \hline
\end{tabular}%

}
% \caption*{ 
% p-value < 0.05 == $\ast$

% p-value < 0.01 == $\ast$$\ast$

% p-value < 0.001 == $\ast$$\ast$$\ast$
% }
\end{table}



% \begin{table}[]
% \caption{}
% \label{tab:my-table}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Programming Language}} & \textbf{Paired t-test normalize paper citation} & \multicolumn{1}{l|}{\textbf{Paired t-test normalize usage coun}} \\ \hline
% Scala      & 0.005360339850403118   & 0.114769451011253   \\ \hline
% C++        & 0.0005684781221390966  & 0.21206043148640416 \\ \hline
% JavaScript & 0.00040948996026648755 & 0.13710897168972622 \\ \hline
% HTML       & 0.0014026359539654441  & 0.09001382882113365 \\ \hline
% OCamel     & 0.0006618795151060018  & 0.03394528878876488 \\ \hline
% Shell      & 0.1328879670060358     & 0.01982989704923204 \\ \hline
% MATLAB     & 0.25428703019620064    & 0.03123284409489575 \\ \hline
% Other      & 0.002890939419679819   & 2.05E-07            \\ \hline
% \end{tabular}%
% }
% \end{table}

==> res/tbl/tbl_programming_languages.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{Percentage of Programming Languages in Paper Artifacts}
\label{tbl_prog_languages}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|c|c|}
\hline
Paper ID &
  \multicolumn{1}{c|}{Paper Title} &
  \textbf{P. Language} &
  \multicolumn{1}{l|}{\textbf{\%}} \\ \hline
9  & Understanding Integer Overflow in C/C++                                                        & C++        & 75.5 \\ \hline
17 & Interface Compliance of Inline Assembly: Automatically Check, Patch and Refine                 & OCamel     & 99.1 \\ \hline
18 & Termination-Checking for LLVM Peephole Optimizations                                           & Shell      & 26.8 \\ \hline
32 & JEST: N+1-version Differential Testing of Both JavaScript Engines and Specification            & Scala      & 97.2 \\ \hline
33 & Data-Oriented Differential Testing of Object-Relational Mapping Systems                        & Scala      & 95   \\ \hline
34 &
  Efficient Detection of Thread Safety Violations via Coverage-Guided Generation of Concurrent Tests &
  Scala &
  76.3 \\ \hline
35 & BigDebug: Debugging Primitives for Interactive Big Data Processing in Spark                    & Scala      & 65.7 \\ \hline
36 & White-Box Performance-Influence Models: A Profiling and Learning Approach                      & Other      & 4.3  \\ \hline
36 & White-Box Performance-Influence Models: A Profiling and Learning Approach                      & Scala      & 44.4 \\ \hline
37 & Efficient Sampling of SAT Solutions for Testing                                                & C++        & 99.7 \\ \hline
38 & Global Optimization of Numerical Programs via Prioritized Stochastic Algebraic Transformations & C++        & 69   \\ \hline
39 & Detecting Incorrect Build Rules                                                                & C++        & 64.8 \\ \hline
40 & Performance regression testing target prioritization via performance risk analysis             & C++        & 60.5 \\ \hline
41 & Efficient construction of approximate call graphs for JavaScript IDE services                  & Javascript & 100  \\ \hline
42 & Poster: Dynamic Analysis Using JavaScript Proxies                                              & Javascript & 100  \\ \hline
43 & Inferring Hierarchical Motifs from Execution Traces                                            & Javascript & 99.6 \\ \hline
44 & Performance Issues and Optimizations in JavaScript: An Empirical Study                         & Javascript & 97.8 \\ \hline
45 & Reasonably-Most-General Clients for JavaScript Library Analysis                                & Javascript & 97.4 \\ \hline
46 & An Empirical Analysis of UI-based Flaky Tests                                                  & HTML       & 100  \\ \hline
47 & A Comparative Study to Benchmark Cross-Project Defect Prediction Approaches                    & HTML       & 97.6 \\ \hline
48 & Multiple-Entry Testing of Android Applications by Constructing Activity Launching Contexts     & HTML       & 96.8 \\ \hline
49 & Automated Repair of Mobile Friendly Problems in Web Pages                                      & HTML       & 87.2 \\ \hline
50 &
  Multi-granular Conflict and Dependency Analysis in Software Engineering Based on Graph Transformation &
  HTML &
  79.2 \\ \hline
51 &
  Avoiding Security Pitfalls with Functional Programming: A Report on the Development of a Secure XML Validator &
  OCamel &
  96.9 \\ \hline
52 & Practical Fault Detection in Puppet Programs                                                   & OCamel     & 96.2 \\ \hline
53 & Poster: Static Analysis of Concurrent Higher-Order Programs                                    & OCamel     & 80.5 \\ \hline
54 & Static Automated Program Repair for Heap Properties                                            & OCamel     & 80.2 \\ \hline
55 & Search-Driven String Constraint Solving for Vulnerability Detection                            & Shell      & 100  \\ \hline
56 & How C++ Developers Use Immutability Declarations: an Empirical Study                           & Shell      & 100  \\ \hline
57 & Brownout: building more robust cloud applications                                              & Shell      & 21.6 \\ \hline
58 & RAICC: Revealing Atypical Inter-Component Communication in Android Apps                        & Shell      & 20.4 \\ \hline
59 &
  SLEMI: Equivalence Modulo Input (EMI) Based Mutation of CPS Models for Finding Compiler Bugs in Simulink &
  MATLAB &
  97.7 \\ \hline
60 &
  Approximation-Refinement Testing of Compute-Intensive Cyber-Physical Models: An Approach Based on System Identification &
  MATLAB &
  39.7 \\ \hline
61 & Automatically Generating Search Heuristics for Concolic Testing                                & Other      & 11.8 \\ \hline
62 & Perses: Syntax-Guided Program Reduction                                                        & Other      & 6    \\ \hline
63 & FAST Approaches to Scalable Similarity-Based Test Case Prioritization                          & Other      & 3.5  \\ \hline
64 & BigDebug: Debugging Primitives for Interactive Big Data Processing in Spark                    & Other      & 3.0  \\ \hline
\end{tabular}%
}
\end{table*}

==> res/tbl/x_tbl_metrics_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%\begin{table*}[]
%\caption{}
%\label{tab:my-table}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{|l|c|c|}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[hbtp]
\caption{Top Five Papers for Usage Attributes}
\label{tbl_top5_papers}
\resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|l|c|c|}
\begin{tabular}{|p{0.04\linewidth}|p{0.5\linewidth}|p{0.15\linewidth}|p{0.08\linewidth}|}
\hline
% \multicolumn{1}{|l|}{Paper ID} &
%   \multicolumn{1}{c|}{\textbf{Paper Title}} &
%   \textbf{Metric} &
%   \multicolumn{1}{l|}{\textbf{Metric Value}} \\ \hline
ID &
Paper Title &
Attribute &
Value \\ \hline
1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Longest Issue                          & 73    \\ \hline
1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Issues Open                            & 48    \\ \hline
1  & Safe Automated Refactoring for Intelligent Parallelization of Java 8 Streams        & Issues Closed                          & 78    \\ \hline
2  & Automated Refactoring of Legacy Java Software to Default Methods                    & Longest Issue                          & 42    \\ \hline
2  & Automated Refactoring of Legacy Java Software to Default Methods                     & Issues Open                            & 47    \\ \hline
2  & Automated Refactoring of Legacy Java Software to Default Methods                    & Issues Closed                          & 113   \\ \hline
3  & Learning Syntactic Program Transformations from Examples                            & Longest Issue                          & 24    \\ \hline
4  & Deep Code Search                                                                    & Stars                                  & 266   \\ \hline
4  & Deep Code Search                                                                    & Paper Citations                        & 134   \\ \hline
4  & Deep Code Search                                                                    & Longest Issue                          & 21    \\ \hline
5 &
  The List is the Process: Reliable Pre-Integration Tracking of Commits on Mailing Lists &
  Longest Issue &
  20 \\ \hline
6  & Feedback-Based Debugging                                                            & Issues Open                            & 54    \\ \hline
6  & Feedback-Based Debugging                                                            & Issues Closed                          & 180   \\ \hline
7  & Accurate and Efficient Refactoring Detection in Commit History                      & Issues Open                            & 34    \\ \hline
7  & Accurate and Efficient Refactoring Detection in Commit History                      & Forks                                  & 121   \\ \hline
7  & Accurate and Efficient Refactoring Detection in Commit History                      & Issues Closed                          & 355   \\ \hline
7  & Accurate and Efficient Refactoring Detection in Commit History                      & Watching                               & 19    \\ \hline
7  & Accurate and Efficient Refactoring Detection in Commit History                      & Stars                                  & 289   \\ \hline
8  & Building and Using Pluggable Type-Checkers                                          & Issues Open                            & 33    \\ \hline
8  & Building and Using Pluggable Type-Checkers                                          & \#Commits & 2290  \\ \hline
8  & Building and Using Pluggable Type-Checkers                                          & Issues Closed                          & 108   \\ \hline
9  & Understanding Integer Overflow in C/C++                                             & Forks                                  & 1700  \\ \hline
9  & Understanding Integer Overflow in C/C++                                             & \#Commits & 40162 \\ \hline
10 & Reducer-Based Construction of Conditional Verifiers                                 & \#Commits & 32527 \\ \hline
% 10 & Reducer-Based Construction of Conditional Verifiers                                 & Watching                               & 21    \\ \hline
% 11 &
%   Code Defenders: Crowdsourcing Effective Tests and Subtle Mutants with a Mutation Testing Game &
%   \#Commits &
%   4464 \\ \hline
% 12 & MU-MMINT: An IDE for Model Uncertainty                                              & \#Commits & 3295  \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Forks                                  & 140   \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Watching                               & 35    \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Stars                                  & 365   \\ \hline
% 13 & Guiding Deep Learning System Testing using Surprise Adequacy                        & Paper Citations                        & 166   \\ \hline
% 14 & On Architectural Diversity of Dynamic Adaptive Systems                              & Watching                               & 20    \\ \hline
% 14 & On Architectural Diversity of Dynamic Adaptive Systems                              & Forks                                  & 1400  \\ \hline
% 15 & DoubleTake: Fast and Precise Error Detection via Evidence-Based Dynamic Analysis    & Watching                               & 18    \\ \hline
% 16 & How Do Developers Fix Cross-Project Correlated Bugs? A Case Study on the GitHub ... & Forks                                  & 214   \\ \hline
% 17 & Interface Compliance of Inline Assembly: Automatically Check, Patch and Refine      & Stars                                  & 244   \\ \hline
% 18 & Termination-Checking for LLVM Peephole Optimizations                                & Stars                                  & 210   \\ \hline
% 19 & Heaps'n Leaks: How Heap Snapshots Improve Android Taint Analysis                    & Artifact Downloads                     & 8388  \\ \hline
% 20 & SOAR: A Synthesis Approach for Data Science API Refactoring                         & Artifact Downloads                     & 3343  \\ \hline
% 21 & Representation of Developer Expertise in Open Source Software                       & Artifact Downloads                     & 2553  \\ \hline
% 22 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                          & Artifact Downloads                     & 1410  \\ \hline
% 22 & FlakeFlagger: Predicting Flakiness Without Rerunning Tests                          & Artifact Views                         & 846   \\ \hline
% 23 & Data clone detection and visualization in spreadsheets                              & Artifact Downloads                     & 849   \\ \hline
% 24 & Automated Reporting of Anti-Patterns and Decay in Continuous Integration            & Artifact Views                         & 5463  \\ \hline
% 25 & Data clone detection and visualization in spreadsheets                              & Artifact Views                         & 1998  \\ \hline
% 26 & Learning from, Understanding, and Supporting DevOps Artifacts for Docker            & Artifact Views                         & 712   \\ \hline
% 27 & Recognizing Developers' Emotions while Programming                                  & Artifact Views                         & 667   \\ \hline
% 28 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars           & Paper Citations                        & 321   \\ \hline
% 28 & DeepTest: Automated Testing of Deep-Neural-Network-Driven Autonomous Cars           & Paper Views                            & 2218  \\ \hline
% 29 & A Novel Neural Source Code Representation based on Abstract Syntax Tree             & Paper Citations                        & 153   \\ \hline
% 29 & A Novel Neural Source Code Representation based on Abstract Syntax Tree             & Paper Views                            & 5704  \\ \hline
% 30 & Semantically Enhanced Software Traceability Using Deep Learning Techniques          & Paper Citations                        & 132   \\ \hline
% 30 & Semantically Enhanced Software Traceability Using Deep Learning Techniques          & Paper Views                            & 3067  \\ \hline
% 31 & Semi-supervised Log-based Anomaly Detection via Probabilistic Label Estimation      & Paper Views                            & 2343  \\ \hline
% 32 & Measuring Program Comprehension: A Large-Scale Field Study with Professionals       & Paper Views                            & 2086  \\ \hline
\end{tabular}%
} 
\end{table}


==> sec_relatedwork.tex <==
Researchers have been sharing their research artifacts such as source code, data, compiled software, and portable systems to run their shared artifacts. 
Undoubtedly, these artifacts support the community to advance the research problems. 
To perceive or improve the quality of these artifacts, several papers have contributed editorial notes~\cite{krishnamurthi2013artifact}, investigated the availability of artifacts~\cite{frachtenberg2022research,heumuller2020publish,stefan2022retrospective}, the effectiveness of providing recognition of artifact evaluation~\cite{flittner2018survey}, the process of artifact evaluation~\cite{hermann2020community}, the linkage of the artifact~\cite{heumuller2020publish}, and the visibility of artifacts~\cite{frachtenberg2022research} in research papers published in different software engineering conference venues. 

Specifically, ~\citeauthor{frachtenberg2022research}~\cite{frachtenberg2022research} have studied the availability of the artifact and the impact of the paper (i.e., citations) for the open artifacts.
% This work also required manual intervention of the authors to identify the artifact links due to the absence of artifact metadata. 
Their work inspected the attributes of authors, conference venue prestige, artifact availability lifespan, and papers' textual attributes excluding artifact usage attributes considered in our work.
To support the program committee and community, \citeauthor{flittner2018survey}~\cite{flittner2018survey} have surveyed the authors of the papers who had artifacts with their papers from CoNEXT, ICN, IMC, and SIGCOMM conferences.
However, these related works provide valuable insight and directions for authors, reviewers, and the community. 
Also, our work goes further than the link and looks into various metadata from various artifact publishing platforms.

We find the most aligned with our work is by 
~\citeauthor{heumuller2020publish}~\cite{heumuller2020publish} reported an empirical study on software artifact papers published at ICSE similar to our venue selection.
The authors investigated types, distributions, and the relationship between artifact availability and paper citations and found a positive correlation between them.
However, they did not consider any additional paper or artifact usage attributes in their research. 
Their work adapted a citation normalization technique~\cite{hutchins2016relative,piwowar2018state}, which normalizes the citation of a paper by the average citation count of all ICSE papers from that year. 
In our case, we normalize the citation with the age of the paper directly because all research papers do not get citations as their co-published papers due to the type of work, size of the community, accessibility to the resources, or the progression rate of the work. 

Another prior work by~\citeauthor{stefan2022retrospective}~\cite{stefan2022retrospective} analyzed the articles mainly focusing on badges and contrasted the presence and types of badges of the artifacts. 
They also tested the relationship between the types of articles for a subset of GitHub attributes, which we have analyzed in this paper.
On the other hand, we exploit the ``Available'' badges for the data collection process and are limited to a single top conference venue, ICSE.
Our work includes the usage attribute from both GitHub and non-GitHub platforms and exclusively compares within and across paper and artifact usage attribute values. 

